Deleting, Eliminating and Decomposing to Hereditary Classes Are All FPT-Equivalent

For a graph class ${\cal H}$, the graph parameters elimination distance to ${\cal H}$ (denoted by ${\bf ed}_{\cal H}$) [Bulian and Dawar, Algorithmica, 2016], and ${\cal H}$-treewidth (denoted by ${\bf tw}_{\cal H}$) [Eiben et al. JCSS, 2021] aim to minimize the treedepth and treewidth, respectively, of the "torso" of the graph induced on a modulator to the graph class ${\cal H}$. Here, the torso of a vertex set $S$ in a graph $G$ is the graph with vertex set $S$ and an edge between two vertices $u, v \in S$ if there is a path between $u$ and $v$ in $G$ whose internal vertices all lie outside $S$. In this paper, we show that from the perspective of (non-uniform) fixed-parameter tractability (FPT), the three parameters described above give equally powerful parameterizations for every hereditary graph class ${\cal H}$ that satisfies mild additional conditions. In fact, we show that for every hereditary graph class ${\cal H}$ satisfying mild additional conditions, with the exception of ${\bf tw}_{\cal H}$ parameterized by ${\bf ed}_{\cal H}$, for every pair of these parameters, computing one parameterized by itself or any of the others is FPT-equivalent to the standard vertex-deletion (to ${\cal H}$) problem. As an example, we prove that an FPT algorithm for the vertex-deletion problem implies a non-uniform FPT algorithm for computing ${\bf ed}_{\cal H}$ and ${\bf tw}_{\cal H}$. The conclusions of non-uniform FPT algorithms being somewhat unsatisfactory, we essentially prove that if ${\cal H}$ is hereditary, union-closed, CMSO-definable, and (a) the canonical equivalence relation (or any refinement thereof) for membership in the class can be efficiently computed, or (b) the class admits a "strong irrelevant vertex rule", then there exists a uniform FPT algorithm for ${\bf ed}_{\cal H}$.

==> PreambleNew.tex <==
\newcommand{\longversion}[1]{{#1}
\newcommand{\shortversion}[1]}

%\usepackage[dvipsnames,svgnames,x11names]{xcolor}
\usepackage{soul}

\usepackage{mdframed}
\usepackage{tcolorbox}

\newcommand{\hlr}[1]{\sethlcolor{Salmon1}\hl{#1}\sethlcolor{yellow}} 
\newcommand{\hlg}[1]{\sethlcolor{PaleGreen2}\hl{#1}\sethlcolor{yellow}}
\newcommand{\hlb}[1]{\sethlcolor{SkyBlue1}\hl{#1}\sethlcolor{yellow}}
\newcommand{\hlo}[1]{\sethlcolor{Apricot}\hl{#1}\sethlcolor{yellow}}
\newcommand{\hly}[1]{\sethlcolor{Gold}\hl{#1}\sethlcolor{yellow}}
\usepackage{listings}
\usepackage{mathrsfs}
\usepackage[mathscr]{euscript}
\usepackage{amsfonts,amsthm,amsmath}
\usepackage{amstext}
\usepackage{graphicx,tikz}
\RequirePackage{fancyhdr}
\usepackage{boxedminipage}
\usepackage[linesnumbered, boxed, algosection,noline]{algorithm2e}
\usepackage{graphics}
\usepackage{pgf}
\usepackage{paralist} 
\usepackage{framed}
\usepackage{thm-restate}
\usepackage{thmtools}
\usepackage{enumerate}
\usepackage{float}
\usepackage{xspace}
\usepackage{todonotes}
\usepackage{tcolorbox}

\usepackage{vmargin}
\setmarginsrb{1in}{1in}{1in}{1in}{0pt}{0pt}{0pt}{6mm}

\newcommand{\myparagraph}[1]{\smallskip\noindent{\textbf{\sffamily #1}}}

\newtheorem{theorem}{Theorem}[section]
\newtheorem{thm}{Theorem}[section]
\newtheorem{lemma}{Lemma}[section]
\newtheorem{claim}[lemma]{Claim}
\newtheorem{corollary}[lemma]{Corollary}
\newtheorem{definition}[lemma]{Definition}
\newtheorem{observation}[lemma]{Observation}
\newtheorem{proposition}[lemma]{Proposition}
\newtheorem{redrule}[lemma]{Reduction Rule}
\newtheorem{remark}[lemma]{Remark}
\newtheorem{reduction}[lemma]{Reduction Rule}
\newtheorem{conjecture}[lemma]{Conjecture}

\date{}
 
%\newcommand{\defparproblem}[4]{
%\vspace{1mm}
%\noindent\fbox{
%  \begin{minipage}{0.96\textwidth}
%  \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lr} #1  & {\bf{Parameter:}} #3 \\ \end{tabular*}
%  {\bf{Input:}} #2  \\
%  {\bf{Question:}} #4
%  \end{minipage}
%}\vspace{1mm}}
%
%\newcommand{\defproblem}[3]{
%\vspace{1mm}
%\noindent\fbox{
%  \begin{minipage}{0.96\textwidth}
%  \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lr} #1 \\ \end{tabular*}
%  {\bf{Input:}} #2  \\
%  {\bf{Question:}} #3
%  \end{minipage}
%}\vspace{1mm}}
%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\usetikzlibrary{decorations.markings}

  \tikzset{vo/.style = {
		shape= circle,
		fill = blue,
		inner sep = 2pt,
		outer sep = 0pt,
		minimum size = 8 pt}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\OO}{\mathcal{O}}
%\newcommand{\cS}{\mathcal{S}}
\newcommand{\yes}{\textsf{Yes}}
\newcommand{\no}{\textsf{No}}
\newcommand{\yesinstance}{\yes-instance}
\newcommand{\noinstance}{\no-instance}
%\newcommand{\tw}{\mathtt{tw}}
\newcommand{\NP}{\textsf{NP}}
\newcommand{\coNP}{\textsf{co-NP}}
\newcommand{\FPT}{\textsf{FPT}}
\newcommand{\XP}{\textsf{XP}}
\newcommand{\WO}{\textsf{W[1]}}
\newcommand{\WOH}{\textsf{W[1]}-hard}
\newcommand{\WOC}{\textsf{W[1]}-complete}
\newcommand{\WTH}{\textsf{W[2]}-hard}
\newcommand{\WTC}{\textsf{W[2]}-complete}
\newcommand{\NPH}{\textsf{NP}-hard}
\newcommand{\NPC}{\textsf{NP}-complete}
\newcommand{\paraH}{\textsf{para-NP}-hard}
\newcommand{\ETH}{\textsf{ETH}}
\newcommand{\SETH}{\textsf{SETH}}
\newcommand{\domain}{\mbox{\sf dom}}
\newcommand{\image}{\mbox{\sf ima}}

\usepackage{booktabs}
\usepackage[pdftex, plainpages = false, pdfpagelabels, 
                 %pdfpagelayout = useoutlines,
                 bookmarks=false,
                 bookmarksopen = true,
                 bookmarksnumbered = true,
                 breaklinks = true,
                 linktocpage,
                 pagebackref,
                 colorlinks = true,  % was true
                 linkcolor = blue,
                 urlcolor  = blue,
                 citecolor = red,
                 anchorcolor = green,
                 hyperindex = true,
                 hyperfigures
                 ]{hyperref}
								
% Paper-specific commands								
\newcommand{\Mark}{\textsf{Mark}}
\newcommand{\mar}{\mbox{\sf mark}}
\newcommand{\vis}{\mbox{\sf vis}}

\newcommand{\cSuccessEnough}{$2$}
\newcommand{\cSuccessStage}{$1$}
\newcommand{\cBigClique}{$10$}
\newcommand{\cHeavyMark}{$3$}
\newcommand{\cVisibleOut}{$1$}
\newcommand{\cVisibleIn}{$1$}

\newcommand{\sm}{\setminus}
%\newcommand{\kk}{{k^{1/2}}}
\newcommand{\kk}{{\sqrt{k}}}
\newcommand{\kkk}{{k^{3/2}}}

\newcommand{\hy}{\widehat{Y}}
\newcommand{\hx}{\widehat{X}}
\newcommand{\hc}{\widehat{C}}
\newcommand{\hs}{\widehat{S}}
\newcommand{\ha}{\widehat{A}}
\newcommand{\la}{\leftarrow}

%% Problem Names 
\newcommand{\vcfull}{{\sc Vertex Cover}\xspace}
\newcommand{\fvstfull}{{\sc Feedback Vertex Set in Tournaments}\xspace}
\newcommand{\fvst}{{\sc FVST}\xspace}
\newcommand{\fvsfull}{{\sc Feedback Vertex Set}\xspace}
\newcommand{\fvs}{{\sc FVS}\xspace}

\newcommand{\dspfull}[1]{$#1$-\text{{\sc Set Packing}}\xspace}
\newcommand{\ddmfull}[1]{$#1$-\text{{\sc Dimensional Matching}}\xspace}
\newcommand{\dhsfull}[1]{$#1$-\text{{\sc Hitting Set}}\xspace}

\newcommand{\dhs}[1]{$#1$-\text{{\sc HS}}\xspace}
\newcommand{\hsetfull}{{\sc Hitting Set}\xspace}
\newcommand{\hset}{{\sc HS}\xspace}


\newcommand{\cvdfull}{{\sc Cluster Vertex Deletion}\xspace}
\newcommand{\cvd}{{\sc CVD}\xspace}

\newcommand{\ippfull}{{\sc Induced $P_3$-Packing}\xspace}
\newcommand{\tptfull}{{\sc Triangle Packing in Tournaments}\xspace}
\newcommand{\tpt}{{\sc TPT}\xspace}

\DeclareMathOperator{\poly}{poly}
\newcommand{\good}{output-parameter sensitive}

==> preamble.tex <==
% Paper specific macros.
\usepackage{mathrsfs}
 \usepackage{amsfonts,amsthm,amsmath}
\usepackage{amstext}
\usepackage{wasysym}
\usepackage{bm}
\usepackage{hyperref}
\usepackage{soul}
\usepackage{xspace}
\usepackage{comment}
\usepackage{tikz}

\usetikzlibrary{shapes.geometric,matrix,shapes,arrows,positioning,chains}
\usepackage[normalem]{ulem}
\usepackage{todonotes}
\usepackage{graphicx,tikz}
\RequirePackage{fancyhdr}
\usepackage{xcolor}
\usepackage{boxedminipage}
\newcommand{\red}[1]{\textcolor{red}{#1}}
%\usepackage[ruled,vlined,linesnumbered]{algorithm2e}

%\newcommand{\compass}{\NP\subseteq \coNP/\poly}

\newcommand{\ncompass}{\NP\nsubseteq \coNP/\poly}
\newcommand{\coNPbypoly}{${\sf co\- NP/Poly}$}
%\newcommand{\coNP}{\text{\normalfont co-NP}}
%\newcommand{\XP}{\text{\normalfont XP}}
%\newcommand{\W}[1][xxxx]{\text{\normalfont W[#1]}}
%\newcommand{\WTH}{\textsf{W[2]}-hard}
%\newcommand{\WTC}{\textsf{W[2]}-complete}
%\newcommand{\NPH}{\textsf{NP}-hard}
%\newcommand{\NPC}{\textsf{NP}-complete}

%\newcommand[1]{\C}{\mathcal{#1}}

%\newcommand{\Yes}{\textsf{yes}}
%\newcommand{\yes}{\textsf{yes}\xspace}
%\newcommand{\No}{\textsf{no}} 
%\newcommand{\no}{\textsf{no}\xspace} 

%%%MZ%%%
%\usepackage{tcolorbox}
%\newcommand{\hlr}[1]{\sethlcolor{red}\hl{#1}\sethlcolor{yellow}} 
%\newcommand{\hlg}[1]{\sethlcolor{green}\hl{#1}\sethlcolor{yellow}}
%\newcommand{\hlb}[1]{\sethlcolor{blue}\hl{#1}\sethlcolor{yellow}}
%\newcommand{\hlo}[1]{\sethlcolor{Apricot}\hl{#1}\sethlcolor{yellow}}
%\newcommand{\hly}[1]{\sethlcolor{Gold}\hl{#1}\sethlcolor{yellow}}
%%%%%%%%

%%%%AA%%%%%%
\newcommand{\C}[1]{\mathcal{#1}}
\newcommand{\what}{\widehat}
\newcommand{\Trun}[2]{{\sf Trun}_{#1}(#2)}
\newcommand{\Degd}{{\cal F}_d}
%%%%%%%%%%%


%\newcommand{\tw}[0]{\mathsf{tw}}
%\newcommand{\td}[0]{\mathsf{td}}


\newcommand{\TW}[1]{\mathcal{T}_{#1}}
%\newcommand{\C}[1]{\mathcal{#1}}
\newcommand{\SC}[1]{\mathscr{#1}}

\newcommand{\powset}[1]{{2}^{#1}}
\newcommand{\Lf}[1]{{\sf Lf}(#1)}
\newcommand{\rt}[1]{{\sf rt}(#1)}
\newcommand{\Pth}[2]{{\sf Pth}_{#1}(#2)}

\newcommand{\ext}{{\sf ext}}
\newcommand{\ath}{{\sf ath}}
%\newcommand{\what}{\widehat}
\newcommand{\wtilde}{\widetilde}
\newcommand{\ns}[1]{[#1]}
\newcommand{\nsz}[1]{[#1]_0}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\mP}{\mathfrak{P}}
\newcommand{\wX}{\what{X}}
\newcommand{\wY}{\what{Y}}
\newcommand{\wW}{\what{W}}
\newcommand{\wF}{\what{F}}
\newcommand{\wf}{\what{f}}
\newcommand{\wg}{\what{g}}

\newcommand{\ump}{{\sf ump}}
\newcommand{\seta}{{\sf cura}}
%\newcommand{\setb}{{\sf curb}}
\newcommand{\setb}{{\sf sep}}
\newcommand{\setap}{{\sf cura'}}
\newcommand{\fillup}{{\sf fill}}
\newcommand{\fillset}{\{\seta,\setb,\setap,\ump\}}


%\newcommand{\ump}{{\sf ump}}
%\newcommand{\cur}{{\sf cur}}
%\newcommand{\setb}{{\sf curb}}
%\newcommand{\rst}{{\sf rst}}
%\newcommand{\fillupone}{{\sf fill}}
%\newcommand{\ump}{{\sf ump}}
\newcommand{\cur}{{\sf alw}}
%\newcommand{\setb}{{\sf curb}}
%\newcommand{\rst}{{\sf rst}}
%\newcommand{\fillupone}{{\sf fill}}

\newcommand{\fillsetnew}{\{\cur,\setb,\ump\}}

\newcommand{\simiso}{{\simeq_{\sf iso}}}

%%%%LQ%%%%

\newcommand{\cB}{\mathcal{B}}

\newcommand{\defparprob}[4]{
  \vspace{1mm}
\noindent\fbox{
  \begin{minipage}{0.96\textwidth}
  \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lr} #1  & {\bf{Parameter:}} #3
\\ \end{tabular*}
  {\bf{Input:}} #2  \\
  {\bf{Question:}} #4
  \end{minipage}
  }
  \vspace{1mm}
}

\newcommand{\defparproblem}[4]{
  \vspace{1mm}
\noindent\fbox{
  \begin{minipage}{0.96\textwidth}
  \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lr} #1  \\ \end{tabular*}
  {\bf{Input:}} #2  \\
  {\bf{Parameter:}} #3\\
  {\bf{Question:}} #4
  \end{minipage}
  }
  \vspace{1mm}
}


\newcommand{\defprob}[3]{
  \vspace{1mm}
\noindent\fbox{
  \begin{minipage}{0.96\textwidth}
  \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lr} #1   \\ \end{tabular*}
  {\bf{Input:}} #2  \\
  {\bf{Question:}} #3
  \end{minipage}
  }
  \vspace{1mm}
}


%\newcommand{\edtdfull}{{\sc Elimination Distance to $\mathcal{H}_d$}\xspace}
%\newcommand{\edtd}{{\sc ED to $\mathcal{H}_d$}\xspace}
%
%\newcommand{\bedtdfull}{{\sc Border Elimination Distance to $\mathcal{H}_d$}\xspace}
%\newcommand{\bedtd}{{\sc BED to $\mathcal{H}_d$}\xspace}

\newcommand{\setp}{{$p$}\xspace}
\newcommand{\setq}{{$q$}\xspace}


\newcommand{\Toposet}[1]{\eta\mbox{-}{\sf TopoSet}{(#1)}}
\newcommand{\Topo}[2]{{\sf Topo}_{#1}(#2)}





%%%%%%%%%%%%%%%%%%LQ2 preamble

%\newcommand{\ak}{{\alpha_k}\xspace}
\newcommand{\ak}{{\alpha (k)}\xspace}
\newcommand{\edtffull}{{\sc Elimination to $\C{H}_\C{F}$}\xspace}
\newcommand{\edtf}{{\sc ED to $\C{H}_\C{F}$}\xspace}

\newcommand{\akku}{{$(\ak,k)$-unbreakable}\xspace}

\newcommand{\uedtffull}{{\sc $\alpha$-Unbreakable Elimination Distance to $\C{H}_\C{F}$}\xspace}
\newcommand{\uedtf}{{\sc $\alpha$-Unbreakable ED to $\C{H}_\C{F}$}\xspace}


\newcommand{\hf}{\mathcal{H}_\mathcal{F}}
\newcommand{\fpt}{{\sc FPT}\xspace}
\newcommand{\fnk}{\psi(k)}

\newcommand{\BB}[1]{{\mathbb #1}}
\newcommand{\lcc}{\ak+1}
\newcommand{\nscc}{\gamma(k)}
\newcommand{\lnscc}{\delta(k)}
\newcommand{\nlccvb}{3(\ak+k)-1}
\newcommand{\anotruntime}{}
\newcommand{\uruntime}{}
%\newcommand{\edmthffull}{$k$-elimination distance}
\newcommand{\mthf}{{$k$-ed modulator to $\hf$}\xspace}

\newcommand{\bigoh}[0]{\mathcal{O}}
%\input{preamble}


\newcommand{\cS}{{\mathcal{S}}}
\newcommand{\cP}{{\mathcal{P}}}
\newcommand{\cV}{{\mathcal{V}}}
\newcommand{\cF}{{\mathcal{F}}}

\newcommand{\X}{{\mathcal{X}}}

\newcommand{\GETS}{\ensuremath{\leftarrow}}
\newcommand{\TO}   {{\bf to }}
\newcommand{\STEP}  {{\bf step }}
%\newcommand{\AND} {{\bf and }}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cI}{\mathcal{I}}
%\newcommand{\cP}{\mathcal{P}}
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cZ}{\mathcal{Z}}

\newcommand{\cD}{\mathcal{D}}
\newcommand{\cU}{\mathcal{U}}
%\newcommand{\cH}{\mathcal{H}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cK}{\mathcal{K}}
%\newcommand{\cP}{\mathcal{P}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cM}{\mathcal{M}}

\newcommand{\bA}{\mathbf{A}}
\newcommand{\bB}{\mathbf{B}}
\newcommand{\bC}{\mathbf{C}}
\newcommand{\bD}{\mathbf{D}}
\newcommand{\bF}{\mathbf{F}}
\newcommand{\bG}{\mathbf{G}}
\newcommand{\bH}{\mathbf{H}}
\newcommand{\bK}{\mathbf{K}}
\newcommand{\bP}{\mathbf{P}}
\newcommand{\bW}{\mathbf{W}}
\newcommand{\bZ}{\mathbf{Z}}
\newcommand{\bX}{\mathbf{X}}

\newcommand{\soldec}{{$(k,\hf)$-decomposition}\xspace}

\newcommand{\solname}{{$(k,\hf)$-topology}\xspace}


%%%%Added by AA%%%%
\newcommand{\scbrksize}{(\ak,k)}
\newcommand{\grsize}{3(\ak+k)} 
\newcommand{\htd}{$\C{H}$-tree decomposition}
\newcommand{\hTD}{$\C{H}$-Tree Decomposition}
\newcommand{\hed}{$\C{H}$-elimination decomposition}
\newcommand{\hED}{$\C{H}$-Elimination Decomposition}
\newcommand{\annhtw}{\textsc{Annotated $\C{H}$-Treewidth}} 
\newcommand{\hhed}[1][\hh]{\ed_{#1}}

\newcommand{\auedtffull}{{\sc $\alpha$-Extension $\C{H}$-Elimination Distance}}

\newcommand{\auedtf}{{\sc $\alpha$-Ext  $\C{H}$-ED}}

\newcommand{\stdst}{$\C{S}_{\sf str}$-tree decomposition}
\newcommand{\sedst}{$\C{S}_{\sf str}$-elimination decomposition}
\newcommand{\ssdepthst}[2][\SSS]{\ed_{{#1}_{\sf #2}}}
\newcommand{\sstwst}[2][\SSS]{\tw_{{#1}_{\sf #2}}}

\newcommand{\hhtwp}[1]{\tw_{#1}}

\newcommand{\hhdepthp}[1]{\ed_{#1}}

\newcommand{\hhmdp}[1]{\md_{#1}}

\newcommand{\hedp}[1]{#1-elimination decomposition}

\newcommand{\htdp}[1]{#1-tree decomposition}

\newcommand{\longobs}{$\dagger$-AW}
\newcommand{\dlongobs}{$\ddagger$-AW}

%%%%%%%%%Added by LQ%
\newcommand{\aedh}{\textsc{$\alpha$-Ext-$\C{H}$-Elimination Distance}\xspace}



